Grokfast: Accelerated Grokking by Amplifying Slow Gradients

One puzzling artifact in machine learning dubbed grokking is where delayed generalization is achieved tenfolds of iterations after near perfect overfitting to the training data. Focusing on the long delay itself on behalf of machine learning practitioners, our goal is to accelerate generalization of a model under grokking phenomenon. By regarding a series of gradients of a parameter over training iterations as a random signal over time, we can spectrally decompose the parameter trajectories under gradient descent into two components: the fast-varying, overfitting-yielding component and the slow-varying, generalization-inducing component. This analysis allows us to accelerate the grokking phenomenon more than $\times 50$ with only a few lines of code that amplifies the slow-varying components of gradients. The experiments show that our algorithm applies to diverse tasks involving images, languages, and graphs, enabling practical availability of this peculiar artifact of sudden generalization. Our code is available at https://github.com/ironjr/grokfast.

==> algorithms/avg.tex <==
\begin{algorithm}[t]
\newcommand{\hlcolor}{OliveGreen}
   \caption{\textsc{Grokfast-MA}}
   \label{alg:avg}
\begin{algorithmic}
   \STATE {\bfseries Input:} initial parameters $\theta_{0}\,$, stochastic objective function $f(\theta)\,$, parameter update $u(g, t)$ from gradient $g$ at timestep $t\,$, e.g., $u$ can be \textsc{SGD}, \textsc{Adam}, etc.
   \STATE {\bfseries Hyperparameter:} {\color{\hlcolor} window size $w\,$, scalar factor $\lambda\,$.}
   \STATE $t \leftarrow 0\,$; {\color{\hlcolor} $Q \leftarrow \mathrm{Queue}(\mathrm{capacity}=w)\,$}: a gradient queue.
   \WHILE {$\theta_{t}$ not converged}
       \STATE $t \leftarrow t + 1$
       \STATE $g_{t} \leftarrow \nabla_{\theta} f(\theta_{t - 1})\,$: Calculate the gradients.
       \STATE {\color{\hlcolor} $\mathrm{Insert}(Q, g_{t})\,$}: Insert the gradients to $Q\,$.
       \STATE {\color{\hlcolor} $\hat{g}_{t} \leftarrow g_{t} + \lambda \cdot  \mathrm{mean}\,(Q)\,$}: Filter the gradients.
       \STATE $\hat{u}_{t} \leftarrow u({\color{\hlcolor} \hat{g}_{t}}, t)\,$: Calculate the parameter update.
       \STATE $\theta_{t} \leftarrow \theta_{t - 1} + \hat{u}_{t}\,:$ Update the parameters.
   \ENDWHILE
\end{algorithmic}
\end{algorithm}

==> figures/result_qm9/main.tex <==
\begin{figure}[t]
\newcommand{\figwidth}{0.495\linewidth}
\begin{center}
\subfloat[\small Loss with respect to amplifier gain $\lambda\,$. \label{fig:qm9:loss_gain}]{\includegraphics[width=\figwidth]{figures/result_ma/grokfast_ma_lambda_loss_v2.pdf}}
\hfill
\subfloat[\small Accuracy with respect to amplifier gain $\lambda\,$. \label{fig:qm9:acc_gain}]{\includegraphics[width=\figwidth]{figures/result_ma/grokfast_ma_lambda_acc_v2.pdf}}
\caption{%
\textbf{Acceleration of delayed generation with \textsc{Grokfast}.}
The amount of acceleration relies on the two hyperparameters, amplifier gain $\lambda$ and window size $w\,$.
% Each hyperparameter has a sweet spot; increasing one arbitrarily does not guarantee faster acceleration.
Figures~\ref{fig:qm9:loss_gain} and~\ref{fig:qm9:acc_gain} uses $\alpha = 100$ except the baseline.
Figures~\ref{fig:qm9:loss_window} and~\ref{fig:qm9:acc_window} uses $\lambda = 5$ except the baseline.
}
\label{fig:qm9}
\end{center}
\vskip -0.2in
\end{figure}

==> macro.tex <==
\newcommand{\ie}{{i.e.}}
\newcommand{\eg}{{e.g.}}
\newcommand{\cf}{{c.f.}}
\newcommand{\etal}{{et al.}}

% \newcommand{\salientcolor}{OliveGreen}
\newcommand{\salientcolor}{BurntOrange}
